What can you do with a rock? Affordance extraction via word embeddings

Autonomous agents must often detect affordances: the set of behaviors enabled by a situation. Affordance detection is particularly helpful in domains with large action spaces, allowing the agent to prune its search space by avoiding futile behaviors. This paper presents a method for affordance extraction via word embeddings trained on a Wikipedia corpus. The resulting word vectors are treated as a common knowledge database which can be queried using linear algebra. We apply this method to a reinforcement learning agent in a text-only environment and show that affordance-based action selection improves performance most of the time. Our method increases the computational complexity of each learning step but significantly reduces the total number of steps needed. In addition, the agent's action selections begin to resemble those a human would choose.

==> excerpts.tex <==
One might question why Wikipedia should be used as a source of common sense knowledge when knowledge bases such as ConceptNet, Cyc, WordNet have been extensively curated to record [num] of linguistic connections between words. However, \cite{mikolov2013a} have shown that the implicit semantic structure in word vectors is comparable to the data contained in curated knowledge bases, especially if [conditions of learning, big data, fast algorithm, etc.]


In this paper we argue that making `sense' can be quantified mathematically

and show that the a prior knowledge provided by affordance detection greatly speeds the learning process.

 , reducing the agent's average search space from [] to [] actions per state.

  Although the agent has no symbol grounding or underlying concept of what each word means, the agent is able maximize its rewards within [x] iterations through the game, a speedup of [y{\%}] over naive Q-learning.
  
  The database is a matrix; database queries are formed as linear algebra operations.
  
  This quality can be represented as a mathematical operation across the vector representations of words in the agent's vocabulary.


Our objective is to reduce the agent's search space by encouraging it to explore only verb/object combinations that seem reasonable according to subjective human standards. We define affordances, or the quality of making `sense', as a mathematical operation across the word vectors for the vocabulary. We say that an affordance exists between a verb $v$ and object $n$ if [uh... terminology stuff goes here.]


Further, let $n(w_i) == True$ $iff$ $w_i$ is a noun and let $v(w_i) == True$ $iff$ $w_i$ is a verb.

and


 and let $o \epsilon N$ be an object encountered by the agent in the simulated environment.
 
 Affordances are inherently dependent on the current situation, and must hence be redefined in different contexts. 
